Random Latent Exploration for Deep Reinforcement Learning

We introduce Random Latent Exploration (RLE), a simple yet effective exploration strategy in reinforcement learning (RL). On average, RLE outperforms noise-based methods, which perturb the agent's actions, and bonus-based exploration, which rewards the agent for attempting novel behaviors. The core idea of RLE is to encourage the agent to explore different parts of the environment by pursuing randomly sampled goals in a latent space. RLE is as simple as noise-based methods, as it avoids complex bonus calculations but retains the deep exploration benefits of bonus-based methods. Our experiments show that RLE improves performance on average in both discrete (e.g., Atari) and continuous control tasks (e.g., Isaac Gym), enhancing exploration while remaining a simple and general plug-in for existing RL algorithms. Project website and code: https://srinathm1359.github.io/random-latent-exploration

==> short_related_works.tex <==
There are two main approaches in RL  for exploration, (a) Randomize the agent by injecting noise thus inducing diverse behavior, and (b) Provide explicit reward bonuses that incentivize the agent to go to novel states. \RLE, bridging the two approaches, injects noise into the agent by adding random latent reward bonuses during training. 

Randomness is the key tool in many exploration strategies in RL.  Perhaps the most popular example is  $\epsilon$-greedy or Boltzmann sampling-based exploration~\cite{mnih2013playing, dann2022guarantees, cesa2017boltzmann, eysenbach2018diversity},  which explores by playing random actions. Entropy regularization~\cite{williams1991function,mnih2016asynchronous}, and MaxEnt RL~\cite{haarnoja2018soft,eysenbach2021maximum, garg2023extreme,hazan2019provably} are other instances of exploration algorithms that utilize randomness, as they explicitly bias towards learning policies that have a high entropy. Another exploration approach is to directly inject noise into the parameters of the policy or value networks, e.g. in off-policy methods ~\cite{fortunato2017noisy}, RLHF with linear MDPs \citep{wu2023making}, online RL in tabular  \citep{osband2016generalization}, and linear MDPs \citep{zanette2020frequentist}. Another line of work includes using Thompson sampling \citep{ thompson1933likelihood, thompson1935theory, russo2018tutorial}, or posterior sampling for exploration \citep{osband2013more, gopalan2015thompson, kveton2021meta, zhang2022feel}, which maintains a posterior distribution over the ground truth model and relies on the uncertainty in the posterior distribution for exploration. Posterior sampling, however, is intractable in practical RL settings due to the need to sample from the extremely complex posterior distribution; Various empirical approaches aim to sample from an approximate posterior instead \citep{li2021hyperdqn,dwaracherla2020hypermodels}, but are unfortunately memory intensive. We note that \RLE is different from these other works as it explores by adding random rewards instead of randomizing over the actions, policies, or models of the environment. 

Exploration by adding explicit reward bonuses is also well studied in both theoretical and applied RL literature. A popular technique is to add novelty-based exploration bonuses that are constructed using prediction errors in transition dynamics ~\cite{pathak2017curiosity,pathak2019self,ramesh2022exploring} or outputs of randomly initialized target network \RND~\citep{burda2018exploration}, etc. Other approaches construct reward bonuses using upper confidence bounds on the uncertainty estimates for the underlying model \citep{auer2008near, vaswani2019old}, using discriminatively trained exemplar models to estimate novelty \citep{fu2017ex2}, or using elliptical potentials when the MDP has a linear parameterization \citep{jin2020provably, zhang2022making, agarwal2020pc}.    \asedit{Unfortunately, these methods often introduce additional components into the learning setups, e.g. additional neural networks for generating bonuses and the associated hyperparameters, which can make learning unstable. In contrast, \RLE is much simpler to deploy as it adds random reward functions that are computed using features from the policy network.} 

\RLE closely resembles the idea of  \textit{Follow The Perturbed Leader} (FTPL) developed in RL theory literature \citep{kveton2019garbage, kveton2019perturbed, kveton2020randomized, rakhlin2016bistro, dai2022follow}. FTPL-based methods explore by adding carefully designed perturbations to the reward function that can guarantee optimism; since the perturbations are closely tied to the underlying modeling assumptions, FTPL-based methods are currently limited to restricted settings like linear bandits, tabular MDPs, etc. In contrast, \RLE simply adds a random reward function sampled from a fixed distribution \(P_z\), and is thus applicable in more practical RL settings. Another major difference is that our method also utilizes \(z\)-conditioned policies and value functions, and thus the randomness is shared amongst the reward function, policy network and value network. 

Finally, there is a long line of work in the theoretical RL literature on developing exploration algorithms that can optimally exploit the structure of the underlying task in model-based RL \citep{ayoub2020model, sun2019model, foster2021statistical}, model-free RL \citep{jin2021bellman, du2021bilinear} and agnostic RL setting \citep{jia2023agnostic},  
however, the focus in these works is on statistical efficiency and the provided approaches are not computationally tractable. 

 

